Object-Oriented Design of Graph Oriented Data Structures

Applied research in graph algorithms and combinatorial structures needs comprehensive and versatile software libraries. However, the design and the implementation of flexible libraries are challenging activities. Among the other problems involved in such a difficult field, a very special role is played by graph classification issues. We propose new techniques devised to help the designer and the programmer in the development activities. Such techniques are especially suited for dealing with graph classification problems and rely on an extension of the usual object-oriented paradigm. In order to support the usage of our approach, we devised an extension of the C++ programming language and implemented the corresponding pre-compiler.

==> classer-decl.tex <==
% Remember to use the lgrind style

\Head{}
\File{classer\-decl.eco}{98}{8}{10}{18:38}{486}
\L{\LB{\K{class}_\V{Graph:}_\K{extensible}}}
\L{\LB{___\{}}
\L{\LB{___.\,.\,.}}
\L{\LB{___\K{extend}_\K{void}_\V{Check\_Add\_Edge}();_\C{}//_An_E-method.}}
\CE{}\L{\LB{___\};}}
\L{\LB{}}
\L{\LB{\K{class}_\V{PlanarGraph:}_\K{dynamic}_\V{Graph}}}
\L{\LB{___\{}}
\L{\LB{___\K{private:}}}
\L{\LB{______\V{PlanarGraph}(_\V{Graph}\&_)_\{.\,.\,.\};__\C{}//_Client_cannot_call_this_constructor.}}
\CE{}\L{\LB{}}
\L{\LB{___\K{public:}}}
\L{\LB{______\K{static}_\K{void}_\V{Test}(\V{Graph}\&_\V{g});_____\C{}//_The_pseudo-constructor_performs_the_instantiation_(if_admissible).}}
\CE{}\L{\LB{______\K{void}_\V{Check\_Add\_Edge}()_\{.\,.\,.\};___\C{}//_Check_if_planarity_is_preserved_and_throw_and_exception_if_needed}}
\CE{}\L{\LB{______\K{int}_\V{Get\_number\_of\_faces}();___}}
\L{\LB{___\};}}


==> classer-usage.tex <==
% Remember to use the lgrind style

\Head{}
\File{classer\-usage.eco}{98}{7}{9}{16:29}{398}
\L{\LB{\index{main}\Proc{main}\V{main}()}}
\L{\LB{____\{}}
\L{\LB{____\V{Graph}_\V{g};}}
\L{\LB{____.\,.\,.}}
\L{\LB{____\V{PlanarGraph::Test}(\V{g});__\C{}//_planarity_test_(using_pseudo-consructor)}}
\CE{}\L{\LB{}}
\L{\LB{____\K{if}_(_\V{g}.\{\V{PlanarGraph}\}_)____\C{}//_is_{'}g{'}_recognized_as_planar?_}}
\CE{}\L{\LB{_________\{}}
\L{\LB{_________\V{cout}_\<\<_\S{}\3g_is_planar,_\#_of_faces=\3\SE{}_}}
\L{\LB{______________\<\<_\V{g}.\{\V{PlanarGraph}\}.\V{Get\_number\_of\_faces}()__\C{}//_classer_method_calling}}
\CE{}\L{\LB{______________\<\<_\V{endl};}}
\L{\LB{_________\}}}
\L{\LB{____\}_\C{}//_all_classers_of_{`}g{'}_are_automatically_destroyed}}
\CE{}

==> extender-usage.tex <==
% Remember to use the lgrind style

\Head{}
\File{extender\-usage.eco}{98}{8}{10}{18:33}{419}
\L{\LB{\index{main}\Proc{main}\V{main}()}}
\L{\LB{_____\{}}
\L{\LB{_____\V{Graph}_\V{G};____\C{}//_A_graph}}
\CE{}\L{\LB{_____.\,.\,.}}
\L{\LB{_________________________\C{}//_Two_labelings____________}}
\CE{}\L{\LB{_____\V{Labeling}_\V{L1}(\V{G});__________________\C{}//_automatic_allocation}}
\CE{}\L{\LB{_____\V{Labeling}*_\V{L2}=_\K{new}_\V{Labeling}(\V{G});___\C{}//_dynamic_allocation}}
\CE{}\L{\LB{_____.\,.\,._\C{}//_use_{`}L1{'}_and_{`}L2{'}_accessing_their_methods_as_usual}}
\CE{}\L{\LB{_____\K{delete}_\V{L2};____\C{}//_A_dynamically_allocated_object_has_to_be_deleted,_as_usual.}}
\CE{}\L{\LB{_____.\,.\,.}}
\L{\LB{_____\}_\C{}//_here_L1_is_deleted_before_G}}
\CE{}
